Observation and Confirmation of Nine Strong Lensing Systems in Dark Energy Survey Year 1 Data

We describe the observation and confirmation of \nbconfirmtext\ new strong gravitational lenses discovered in Year 1 data from the Dark Energy Survey (DES). We created candidate lists based on a) galaxy group and cluster samples and b) photometrically selected galaxy samples. We selected 46 candidates through visual inspection and then used the Gemini Multi-Object Spectrograph (GMOS) at the Gemini South telescope to acquire spectroscopic follow-up of 21 of these candidates. Through analysis of this spectroscopic follow-up data, we confirmed nine new lensing systems and rejected 2 candidates, but the analysis was inconclusive on 10 candidates. For each of the confirmed systems, we report measured spectroscopic properties, estimated \einsteinradiussub, and estimated enclosed masses. The sources that we targeted have an i-band surface brightness range of iSB ~ 22 - 24 mag arcsec^2 and a spectroscopic redshift range of zspec ~0.8 - 2.6. The lens galaxies have a photometric redshift range of zlens ~ 0.3 - 0.7. The lensing systems range in image-lens separation 2 - 9 arcsec and in enclosed mass 10^12 - 10^13 Msol.

==> authors_collaboration_apj.tex <==


\author{T.~M.~C.~Abbott}
\affiliation{Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile}
\author{S.~Allam}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{J.~Annis}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{S.~Avila}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{K.~Bechtol}
\affiliation{LSST, 933 North Cherry Avenue, Tucson, AZ 85721, USA}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{D.~Brooks}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{D.~L.~Burke}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{A.~Carnero~Rosell}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~Carrasco~Kind}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{J.~Carretero}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{C.~E.~Cunha}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{L.~N.~da Costa}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{C.~Davis}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{J.~De~Vicente}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{P.~Doel}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{T.~F.~Eifler}
\affiliation{Department of Astronomy/Steward Observatory, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{A.~E.~Evrard}
\affiliation{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{E.~Fernandez}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{B.~Flaugher}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{P.~Fosalba}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{J.~Frieman}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{J.~Garc\'ia-Bellido}
\affiliation{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\author{E.~Gaztanaga}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{D.~Gruen}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{R.~A.~Gruendl}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{G.~Gutierrez}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{W.~G.~Hartley}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\affiliation{Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland}
\author{D.~L.~Hollowood}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{K.~Honscheid}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{B.~Hoyle}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affiliation{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
\author{D.~J.~James}
\affiliation{Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA}
\author{K.~Kuehn}
\affiliation{Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia}
\author{N.~Kuropatkin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{O.~Lahav}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{M.~Lima}
\affiliation{Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~A.~G.~Maia}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~March}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{J.~L.~Marshall}
\affiliation{George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
\author{P.~Melchior}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\author{F.~Menanteau}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{R.~Miquel}
\affiliation{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{A.~A.~Plazas}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{A.~K.~Romer}
\affiliation{Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
\author{A.~Roodman}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{E.~S.~Rykoff}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{E.~Sanchez}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{V.~Scarpine}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{R.~Schindler}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{M.~Schubnell}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{I.~Sevilla-Noarbe}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{M.~Smith}
\affiliation{School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK}
\author{M.~Soares-Santos}
\affiliation{Brandeis University, Physics Department, 415 South Street, Waltham MA 02453}
\author{F.~Sobreira}
\affiliation{Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{E.~Suchyta}
\affiliation{Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831}
\author{M.~E.~C.~Swanson}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{G.~Tarle}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{D.~Thomas}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{Y.~Zhang}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}


\collaboration{(DES Collaboration)}




==> authors_collaboration_mnras.tex <==


\author{T.~M.~C.~Abbott}
\affiliation{Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile}
\author{S.~Allam}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{J.~Annis}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{S.~Avila}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{K.~Bechtol}
\affiliation{LSST, 933 North Cherry Avenue, Tucson, AZ 85721, USA}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{D.~Brooks}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{D.~L.~Burke}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{A.~Carnero~Rosell}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~Carrasco~Kind}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{J.~Carretero}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{C.~E.~Cunha}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{L.~N.~da Costa}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{C.~Davis}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{J.~De~Vicente}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{P.~Doel}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{T.~F.~Eifler}
\affiliation{Department of Astronomy/Steward Observatory, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{A.~E.~Evrard}
\affiliation{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{E.~Fernandez}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{B.~Flaugher}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{P.~Fosalba}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{J.~Frieman}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\author{J.~Garc\'ia-Bellido}
\affiliation{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\author{E.~Gaztanaga}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{D.~Gruen}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{R.~A.~Gruendl}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{G.~Gutierrez}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{W.~G.~Hartley}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\affiliation{Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland}
\author{D.~L.~Hollowood}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{K.~Honscheid}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{B.~Hoyle}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affiliation{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
\author{D.~J.~James}
\affiliation{Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA}
\author{K.~Kuehn}
\affiliation{Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia}
\author{N.~Kuropatkin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{O.~Lahav}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{M.~Lima}
\affiliation{Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~A.~G.~Maia}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~March}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{J.~L.~Marshall}
\affiliation{George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
\author{P.~Melchior}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\author{F.~Menanteau}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{R.~Miquel}
\affiliation{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{A.~A.~Plazas}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{A.~K.~Romer}
\affiliation{Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
\author{A.~Roodman}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{E.~S.~Rykoff}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{E.~Sanchez}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{V.~Scarpine}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{R.~Schindler}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{M.~Schubnell}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{I.~Sevilla-Noarbe}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{M.~Smith}
\affiliation{School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK}
\author{M.~Soares-Santos}
\affiliation{Brandeis University, Physics Department, 415 South Street, Waltham MA 02453}
\author{F.~Sobreira}
\affiliation{Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{E.~Suchyta}
\affiliation{Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831}
\author{M.~E.~C.~Swanson}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{G.~Tarle}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{D.~Thomas}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{Y.~Zhang}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}


\collaboration{(DES Collaboration)}




==> authors_first_apj.tex <==
%\altaffiltext{1}{B.N. email: nord@fnal.gov}
\correspondingauthor{B.~Nord}
\email{nord@fnal.gov}


%\def \ucl {Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
%\def \rhodes {Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa}

\author{B.~Nord}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}

\author{E.~Buckley-Geer}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{H.~Lin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{N.~Kuropatkin}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{T.~Collett}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}

\author{D.~Tucker}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{H.~T.~Diehl}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}

\author{A.~Agnello}
\affiliation{European Southern Observatory, Karl-Schwarzschild-Strasse 2, 85748 Garching, Germany}

\author{A.~Amara}
\affiliation{Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland}




%\author{F.~Ostrovski}\affiliation{\fnal}
%\author{The DES Collaboration}
%F.~B.~Abdalla\altaffilmark{\ucl,\rhodes},
%M.~Auger\altaffilmark{20},
%R.~J.~Brunner\altaffilmark{21,22},
%M.~Carrasco~Kind\altaffilmark{21,22},
%F.~J.~Castander\altaffilmark{23},
%C.~E.~Cunha\altaffilmark{15},
%L.~N.~da Costa\altaffilmark{24,25},
%R.~J.~Foley\altaffilmark{21,26},
%D.~W.~Gerdes\altaffilmark{27},
%K.~Glazebrook\altaffilmark{28},
%J.~Gschwend\altaffilmark{24,25},
%W.~Hartley\altaffilmark{\eth},
%R.~Kessler\affiliation{\kicp},
%D.~Lagattuta\altaffilmark{29},
%G.~Lewis\altaffilmark{30},
%M.~A.~G.~Maia\altaffilmark{24,25},
%F.~Menanteau\altaffilmark{21,22},
%D.~Scolnic\affiliation{\kicp}

% % ... Folks who reviewed images in SV
% % 
% % S.~Allam\affiliation{\fnal},
% % G.~B.~Caminha\altaffilmark{5,6},
% % C.~De Bom\altaffilmark{5,7},
% % S.~Desai\altaffilmark{8,9},
% % H.~D\'umet-Montoya\altaffilmark{10},
% %  M.~Elidaiana da S. Pereira\altaffilmark{5},
% % D.~A.~Finley\affiliation{\fnal},
% % B.~Flaugher\affiliation{\fnal},
% % C.~Furlanetto\altaffilmark{11},
% % S.~Birrer\altaffilmark{3},

% % M.~Gill\altaffilmark{12},
% % K.~W.~Merritt\affiliation{\fnal},
% % A.~More\altaffilmark{13},


% % ... from previous paper
% % A.~Saro\altaffilmark{14},
% % E.~S.~Rykoff\altaffilmark{15,12},
% % E.~Rozo\altaffilmark{16},
% % J.~D.~Vieira\altaffilmark{21,26,22},
% % R.~Gramillano\altaffilmark{21},

% % ... Builders
% % T. M. C.~Abbott\altaffilmark{32},
% % M.~Banerji\altaffilmark{20,33},
% % A.~Benoit-L{\'e}vy\altaffilmark{34,17,35},
% % D.~Brooks\altaffilmark{17},
% % D.~L.~Burke\altaffilmark{15,12},
% % D.~Capozzi\altaffilmark{4},
% % A.~Carnero~Rosell\altaffilmark{24,25},
% % J.~Carretero\altaffilmark{23,36},
% % C.~B.~D'Andrea\altaffilmark{4,37},
% % J.~P.~Dietrich\altaffilmark{8,9},
% % P.~Doel\altaffilmark{17},
% % A.~E.~Evrard\altaffilmark{38,27},
% % J.~Frieman\altaffilmark{1,2},
% % E.~Gaztanaga\altaffilmark{23},
% % D.~Gruen\altaffilmark{39,40},
% % K.~Honscheid\altaffilmark{41,42},
% % D.~J.~James\altaffilmark{32},
% % K.~Kuehn\altaffilmark{43},
% % T.~S.~Li\altaffilmark{44},
% % M.~Lima\altaffilmark{45,24},
% % J.~L.~Marshall\altaffilmark{44},
% % P.~Martini\altaffilmark{41,46},
% % P.~Melchior\altaffilmark{41,47,42},
% % R.~Miquel\altaffilmark{48,36},
% % E.~Neilsen\affiliation{\fnal},
% % R.~C.~Nichol\altaffilmark{4},
% % R.~Ogando\altaffilmark{24,25},
% % A.~A.~Plazas\altaffilmark{49},
% % A.~K.~Romer\altaffilmark{50},
% % M.~Sako\altaffilmark{51},
% % E.~Sanchez\altaffilmark{52},
% % V.~Scarpine\affiliation{\fnal},
% % M.~Schubnell\altaffilmark{27},
% % I.~Sevilla-Noarbe\altaffilmark{52,21},
% % R.~C.~Smith\altaffilmark{32},
% % M.~Soares-Santos\affiliation{\fnal},
% % F.~Sobreira\altaffilmark{1,24},
% % E.~Suchyta\altaffilmark{51},
% % M.~E.~C.~Swanson\altaffilmark{22},
% % G.~Tarle\altaffilmark{27},
% % J.~Thaler\altaffilmark{26},
% % A.~R.~Walker\altaffilmark{32},
% % W.~Wester\affiliation{\fnal},
% % Y.~Zhang\altaffilmark{27}


%\affil{$^{4}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
%\affil{$^{6}$ Dipartimento di Fisica e Scienze della Terra, Universit\`a degli Studi di Ferrara, Via Saragat 1, I-44122 Ferrara, Italy}
%\affil{$^{7}$ Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Rodovia M\'ario Covas, lote J2, quadra J, Cep 23810-000,  Itagua\'i, RJ, Brazil}
%\affil{$^{8}$ Excellence Cluster Universe, Boltzmannstr.\ 2, 85748 Garching, Germany}
%\affil{$^{9}$ Faculty of Physics, Ludwig-Maximilians University, Scheinerstr. 1, 81679 Munich, Germany}
%\affil{$^{10}$ Universidade Federal do Rio de Janeiro - Campus Maca\'e, Rua Alo\'isio Gomes da Silva, 50 - Granja dos Cavaleiros, Cep: 27930-560, Maca\'e, RJ, Brazil}
%\affil{$^{11}$ University of Nottingham, School of Physics and Astronomy, Nottingham NG7 2RD, UK}
%\affil{$^{12}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
%\affil{$^{13}$ Kavli IPMU (WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
%\affil{$^{14}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}
%\affil{$^{15}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
%\affil{$^{16}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA}
%\affil{$^{17}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
%\affil{$^{18}$ Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa}
%\affil{$^{19}$ Department of Physics and Astronomy, PAB, 430 Portola Plaza, Box 951547, Los Angeles, CA 90095-1547, USA}
%\affil{$^{20}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
%\affil{$^{21}$ Department of Astronomy, University of Illinois, 1002 W. Green Street, Urbana, IL 61801, USA}
%\affil{$^{22}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
%\affil{$^{23}$ Institut de Ci\`encies de l'Espai, IEEC-CSIC, Campus UAB, Carrer de Can Magrans, s/n,  08193 Bellaterra, Barcelona, Spain}
%\affil{$^{24}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
%\affil{$^{25}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
%\affil{$^{26}$ Department of Physics, University of Illinois, 1110 W. Green St., Urbana, IL 61801, USA}
%\affil{$^{27}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
%\affil{$^{28}$ Centre for Astrophysics \& Supercomputing, Swinburne University of Technology, Victoria 3122, Australia}
%\affil{$^{29}$ Centre de Recherche Astrophysique de Lyon, Universit\'e de Lyon, Universit\'e Lyon 1, CNRS, Observatoire de Lyon; 9 avenue Charles Andr\`e, 69561 Saint-Genis Laval Cedex, France}
%\affil{$^{30}$ Sydney Institute for Astronomy, School of Physics A28, The University of Sydney, NSW 2006, Australia}
%\affil{$^{31}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus OH 43210, USA}
% %\affil{$^{32}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile}
% %\affil{$^{33}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
% %\affil{$^{34}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
% %\affil{$^{35}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
% %\affil{$^{36}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
% %\affil{$^{37}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK}
% %\affil{$^{38}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
% %\affil{$^{39}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
% %\affil{$^{40}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
% %\affil{$^{41}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
% %\affil{$^{42}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
% %\affil{$^{43}$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia}
% %\affil{$^{44}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
% %\affil{$^{45}$ Departamento de F\'{\i}sica Matem\'atica,  Instituto de F\'{\i}sica, Universidade de S\~ao Paulo,  CP 66318, CEP 05314-970, S\~ao Paulo, SP,  Brazil}
% %\affil{$^{46}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA}
% %\affil{$^{47}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
% %\affil{$^{48}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
% %\affil{$^{49}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
% %\affil{$^{50}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK}
% %\affil{$^{51}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
% %\affil{$^{52}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}





==> extras.tex <==
% links and others
%\slugcomment{Draft for Internal Review: \\ \pubnumdes \\ \pubnumfnal} % slug comment
% https://cdcvs.fnal.gov/redmine/projects/des-stronglens/wiki/SelectedGeminiTargetList2015B
%\documentclass[iop]{emulateapj}
%\documentclass[iop]{aastex61}
%\documentclass[twocolumn]{aastex61}



% ================================================================================
% ================================================================================
% ABSTRACT

% a sample identified in a catalog-based search \citep{diehl17}

% ================================================================================
% ================================================================================
% INTRO

%\citet{diehl17pub} performed a catalog-based photometry search of the $\sim1800$\sqdegadjective\ Y1 area, identifying 374 candidates. 

%With the anticipated dramatic increase in the number of these systems in upcoming surveys, so will come increased power in constraining cosmological parameters. For example 
%With larger numbers of objects, we can refined our measurements via time delays and double source-plane lenses. Moreover, with orders of magntidue more objects, we can With large numbers of galaxy-scale lenses we can also study the galaxy-scale lens mass distribution .

%\begin{itemize}
%\item galaxy evolution
%\item cluster scale measurements
%\item Time delay measurements
%\item double source-plane lenses
%\item image separation distribution
%\end{itemize}
%Additionally, DES may observe over a hundred lensed quasars, a few lensed supernovae and LSST an order of magnitude more \citep{oguri10}.
%, DES has discovered and confirmed two lensed quasars  so far at $z\sim1.6$ and $\sim2.4$ \citep{agnello15}.

%Lens searches, this lens search, and how it may affect future confirmation efforts.

% Agree with Huan's comment here regarding galaxy-scale versus group and cluster

% ================================================================================
% ================================================================================
% Subsection on Data

%Other DESDM refs?



% ================================================================================
% ================================================================================
% Subsection on Lens search


%SPT, redmapper (l >20), redmagic search (color cuts below), and photometric catalog searches (detiled in diehl et al) that were in progress at the time produced a number of candidates. These were scanned by seven? expert scanners and found visually compelling evidence (morphology and photometry): This visual scan resulted in \nbcandidate\ high-ranking candidates. This ranking is distinct from those that are eventually reported in diehl2017.

%The catalog-based algorithms search for objects based on the proximity of candidate sources and lenses, as well as empirically based photometry thresholds. These are categorized into five algorithms --- \BNA, \RNA, SPT, \onek, and \redm. For each of our confirmed systems discussed in \S~\ref{sec:sample}, we first note the original process through which it was discovered, adn then we note the relevant section in the diehl et al paper for which there is additional information on that system. The \redm-identified systems are from searches of \redmagic\ \citep{Elvinpoole17} and \redmapper\ \citep{McClintock17} systems. For detailed descriptions of all of these algorithms, please see \citet{diehl17pub}. 

%Through a set of photometric, spatial cuts and visual scans we identified a candidate sample.

%In this paper, we carried out lens modeling on three galaxy-scale lenses discovered in the Y1A1 data: DESJ0104-5341, DESJ0120-5143 and DESJ2321-4630. The search process that produced the three lenses described in the paper is described in detail in \citet{Diehl2017}. Two of the systems, DESJ0120-5143-4630 and DESJ0104-5341, were first identified in the visual scan of 7328 galaxy clusters identified by the redMaPPer galaxy clustering algorithm \citep{Rykoff2014} in the DES Year 1 data release (Y1A1). The other system, DESJ2321-4630 was identified in a sample of DES year 1 luminous red galaxies selected using the redMaGiC algorithm \citep{Rozo2015} in associated with three or more nearby blue objects, where blue is defined as $-1 \leq g-r < 1$ and $-1 \leq r-i < 1$ and $r < 22$.  Two of the systems, DESJ0120-5143 and DESJ2321-4630 were also identified by the catalog search techniques described in \citet{Diehl2017}. 

%The DES image analysis pipeline measures properties of objects, classifies them as galaxies or stars and populates a database with properties of position, photometry and redshift. 

%\redmapper, \redmagic\ and \onek

%After the catalogs of objects were searched, we proceeded with a visual inspection by half a dozen experienced inspectors. This resulted in \nbcandidate\ high-ranking candidates.

%In \citet{diehl17pub}, the authors searched the Master Lens Database \citep{leonidas16}\footnote{\url{masterlens.astro.utah.edu}} to ascertain if any of the candidates had been previously discovered.

% We actually took data for \nbfollowup.
% (one object was an already confirmed QSO from Fernanda that we took a better spectrum of)


% ================================================================================
% ================================================================================
% Subsection on Observing strategy
%Each 1-hour observing sequence, we observe the lensing system and perform one set of calibrations (flat fields and spectral calibration), then repeat the calibrations and observe the lensing system again. 
%Of the \nbcandidate\ observed candidate systems, we followed up \nbfollowup\ systems. \nbpriorityvisitor\ systems were observed in Priority Visiting observer mode in October and December 2015, and \nbqueuetext\ systems were observed in queue mode in January, February, and December 2016. For \nbdatacomplete\ systems, we obtained all the planned exposures, and for \nbdatapartial\ systems, we obtained a subset of the planned exposures. 

% ================================================================================
% ================================================================================
% Section on Spectroscopic follow-up

%determine if a sample of candidate lensing systems are spectroscopically confirmed, and then to analyze those which are confirmed. 
%\nord{Liz: I think we have 25 objects in total that we followed up, 4 QSO systems 21 galaxy systems. We rejected 2 of the QSO systems and two of the galaxy systems.}
%See \citet{ostrovski17}, and \citet{lin17} for a discussion of two of the successfully confirmed QSO systems. %(Check which of our 21 were quasar systems: use the gemini report sheet)
%which would allow us to detect sources at $z > 2.0$ that produce \Lya\ emission.

% and 2D fits on the calibration data and sky subtraction on the science data, respectively, for individual extensions. 


% ================================================================================
% ================================================================================
% System A
% that may account for the slightly bluer color in this arc than in \arcB\ and \arcC.


% ================================================================================
% ================================================================================
% System D

%\SystemD\ is a small group, where the central lensing galaxy has a photometric redshift of $\zlens=\redshiftlensD$. There is a red arc (\arcA) to the west, a large red arc (\arcB) to the southwest, and a red arc (\arcC) to the south, respectively, as shown in Fig.~\ref{fig:multipanel}d and in Fig.~\ref{fig:SystemD}, top and bottom right panels. In the follow-up R400 spectroscopy of all three arcs (Fig.~\ref{fig:SystemD}, left panels), we identify emission lines near $\sim7141$\AA\ and $\sim8316$\AA, which we identify as \OIIdoublet\ and H$\gamma$, respectively. Also, in arcs \arcA\ and \arcB, we identify a strong emission lines near an observed wavelength of $\sim9567$\AA, which, in the absence of features in the B600 spectra, we take to be \OIIIa. From this pattern of emission lines, we obtain redshifts of $\zsrc=\redshiftsrcDA$, $\redshiftsrcDB$, and $\redshiftsrcDC$ (Fig.~\ref{fig:SystemD}). The red 'x' near the center of the color image in the upper right panel marks the lensing galaxy designated for measurement of the Einstein radius.


% ================================================================================
% ================================================================================
% System I
%\nord{This is a group-scale system.}
%For mask 11 it seems we missed a possible confirmation from the 2015B observations.
%There is a strong emission line in the red data for the second slit, which targeted the blue knot at the end of the arc in this system.  
%If 3727, then the redshift is 1.2525, and the line is seen in both the 2015B and 2016B data.  
%The first slit targets a red object, which looks like a galaxy in the lensing group/cluster and I don't get a redshift from any of the data. 
%Also, the arc in this system is targeted, split between the first two slits, but I don't think I can measure a redshift for the arc. 
%In particular, the line at z = 1.2525 is not seen for the arc in the first slit in the red for the better quality 2016B data. 
%So I think we just get a redshift for the blue knot in this system, and not the arc, but maybe this is good enough to count as a confirmation, %assuming that there wasn't enough S/N in the arc to see the emission line.
%I used the set from Dec 2016 to do the redshift determination as the seeing was much better.
%The line is [OII] at 8396
%The redshift is 1.2526+-0.0001
% Einstein radius is 4.11+-0.28
% Photo-z of lens 0.43+-0.04 however it will have a redmapper redshift
% This system was found with the \redm\ and the \RNA\ algorithms.


% ================================================================================
% ================================================================================
% Discussion

%Many of our unconfirmed systems exhibit clear lensing features but have no detectable continuum or spectral features, with integration times of about $1$ hour on an $8$m-class telescope\footnote{For a number of the targets, we did not obtain the 3.7-hour GMOS R400 observations, which might have helped to confirm more systems.}. The need for long integration time highlights the challenge of obtaining spectra for faint objects found by deep optical surveys, like DES: the challenge will only be greater for the Large Synoptic Survey Telescope\footnote{\url{http://www.lsst.org/lsst/}} \citep[LSST;][]{LSST09}. One faces the prospect of long integration times, which limits the number of systems that can be followed up with a typical program. For systems that exhibit a clear lensing morphology and that have detectable continuum emission but no visible features, IR data may be necessary to confirm them.


%refer to Nordetal2016 for the discussion on telescopes. We will need targeted methods to get the lenses we want for specific science, and we'll want methods to analyze the selection precisely.

%We perform rudimentary modeling, while another paper will provide detailed modeling of some of the systems.

%What will we do lens confirmations in the future?



% ================================================================================
% ================================================================================
% Conclusions

%{\bf We note that two systems from \cite{diehl17} (DESJ2251-4412 and DESJ0538-4022) were followed up with IMACS multi-object spectrograph at the Magellan/Baade Telescope \citep{2006SPIE.6269E..0FD} and were rejected \citep{privatemagellan}.}

%In this paper, we presented the first confirmed group- and cluster-scale strong lensing systems found in DES data. These systems were discovered through visual identification using both targeted and \opensearch\ searches. We confirmed these systems with a combination of spectroscopy from GMOS on the Gemini South telescope and IMACS on the Magellan/Baade telescope.

%Two of these systems are of particular interest, because they have source galaxies at redshifts  $z=2.7251$ and $z=3.22086$. Due to the magnification provided by lensing, these sources are typically among the brightest galaxies in their redshift ranges and can provide an important window into the star formation history and galaxy formation at these cosmic epochs. 

%The candidate lensing systems discovered in DES SV data span a range of arc sizes, much like the currently known sample of candidates from searches during the last decade. Due to the seeing limitations of DES (median expected seeing $\sim 0.9\arcsec $, systems with smaller arc separations were more difficult to identify, especially during the non-targeted search. Thus, our visual inspection methods likely yielded higher completeness in the targeted search of  \redmapper\ and SPT clusters. 

%The candidate lensing systems discovered in DES SV data span a range of arc sizes, much like the currently known sample of candidates from searches during the last decade. Due to the seeing limitations of DES (median expected seeing $\sim 0.9\arcsec $, systems with smaller arc separations were more difficult to identify, especially during the non-targeted search. Thus, our visual inspection methods likely yielded higher completeness in the targeted search of  \redmapper\ and SPT clusters. 

%From improved search methods, like machine learning, we will have better measures of confidence of a lens classification. What does this potentially mean for confirmations?

%If the expected number of lensing systems are discovered in DES and LSST, there will need be a more well-defined focus on the kinds of lenses that are followed up spectroscopically. That is, with the scarcity of follow-up resources, it behooves the community to target those that are maximally beneficial for science cases, such as double source-plane and time-delay lenses.

%Machine learning provide a probability, which may quell the need for confirmation. This may be one of the principal ways in which take advantage of such large data sets. 

%This will likely include searches for the kinds of lenses with which we can do the best science. From improved search methods, like machine learning, we will have better measures of confidence of a lens classification. What does this potentially mean for confirmations?

%, as opposed to just looking for all the lenses possible, though there is some power in understanding the completeness and purity of lenses.







% ================================================================================
% ================================================================================

% Acknowledgments
% C. De Bom would like to thank CNPq for the financial support.

% R.J.F. gratefully acknowledges support from the Alfred P. Sloan Foundation.

% C. Furlanetto acknowledges funding from CAPES (proc. 12203-1). 

==> repository.tex <==
% : 
% \begin{itemize}
% \item R1: $i_{\rm SB} < 23\, {\rm mag}/\sqarcsec$ (six candidates)
% \item R2: $23 < i_{\rm SB} < 24\, {\rm mag}/\sqarcsec$ (14 candidates)
% \item R3: $i_{\rm SB} >24\, {\rm mag}/\sqarcsec$ (four candidates)
% \end{itemize}
% These rankings are not related to the quality rankings of candidates in \S\ref{sec:search}. Details of the observing parameters and conditions for each of our confirmed lensing systems are shown in Table~\ref{table:observationlog}.  17 systems were observed at Gemini and five at Magellan. One of the systems, AAA, was observed at both Gemini and Magellan: only B600 data were acquired at Gemini, which presented no spectral features, so we observed at longer wavelengths at Magellan. 


% \begin{itemize}
% \item R1: 1-hour integration with R150/GG455 grating/filter. 
% \item R2: 1-hour integration with B600 grating and 3.7-hour integration with R150/GG455 grating/filter.
% \item R3: 1-hour integration with B600 grating.
% \end{itemize}



%Thanks to the entire Las Campanas Observatory staff for their help in the acquisition of the Magellan/IMACS data \citep[Inamori Magellan Areal Camera and Spectrograph;][]{bigelow03}. This paper includes data gathered with the 6.5m Magellan Telescopes located at Las Campanas Observatory, Chile.



% One of the main objectives of the strong lensing science program in DES is to derive constraints on dark energy. One of the two key components will be exploiting galaxy- and cluster-scale lenses that have multiple background sources at different redshifts. When there exist two lensed sources, one source will lie between the lens and the other, more distant source: these sources produce distinct Einstein radii. The ratio of the Einstein radii (and thus, a ratio of angular diameter distances) is independent of the Hubble constant, and only weakly dependent on the lens mass distribution.  Provided the lensing mass can be well modeled, the ratio of distance ratios can help to constrain dark energy models \citep{gavazzi08, jullo10, collett12, collett14}. 

% The second key component is to use strongly lensed quasars to measure cosmological parameters (e.g., $ H_0$) by utilizing the time delays between multiple images \citep{refsdal64,suyu13,birrer15} of time-varying sources.   We predict that the wide-field survey should contain about 120 lensed quasars brighter than $i = 21$ mag \citep{oguri10}, of which $\sim20$ would be high-information content quadruple-image configurations. Through the STRong-lensing Insights into Dark Energy Survey (STRIDES) program\footnote{\url{http://strides.physics.ucsb.edu/}}, DES has discovered and confirmed two lensed quasars  so far at $z\sim1.6$ and $\sim2.4$ \citep{agnello15}. In addition, 30~\sqdeg\ of deep imaging in the supernova fields, which have a high cadence, provides an opportunity to find lensed supernovae.

% In addition to constraining cosmology, we will use a substantial cluster-scale lens sample to study dark matter mass profiles. Also, we expect to discover a large sample of sources at varying redshifts that will be valuable for studies of galaxy evolution.


%In total, SV observations cover $\sim 250$ \sqdeg\ in five optical filter bands ($grizY$), nearly reaching the expected full five-year depth of DES: below, we report median depth estimates of these data at $10\sigma$ galaxy limiting magnitude. The wide-field survey consists of the SPT-E and SPT-W fields that are located, respectively, in the east and west regions of the South Pole Telescope (SPT) survey footprint \citep{carlstrom11}: the $g$-band depth extends to $\sim 24.5$ mag. The $30$\sqdegadjective\ supernova survey takes place in eight shallow fields, and two deep fields, extending to $g$-band depths, $25.0$ mag and $25.4$ mag, respectively.






%future higher-resolution imaging follow-up may allow for detailed modeling of cluster mass distributions.

%\begin{rewrite}The Year 1 DES data cover an area of $\sim1800$ \sqdeg, and we have already conducted targeted searches, identifying a number of promising systems for follow-up.  catalog-based photometry searches similar to those employed in the SBAS \citep[e.g.,][]{diehl09}. We continue the dedicated program, STRIDES \citep{treu15}, to search for lensed quasars. With these tools, our searches through Year 1 data will be more effective than in SV for finding galaxy-scale lenses. \end{rewrite}

%General Relativity's canonical maxim was coined by John Wheeler: "Matter tells space-time how to curve, and space-time tells matter how to move." 


%Strong lensing also provides a sample of galaxies---the lenses themselves---that are selected based on total mass, rather than luminosity or surface brightness  \citep[e.g.,][]{reblinsky99}: the distortion of images by the lens  depends only on the total lens mass and its spatial distribution.%\footnote{This is not the case for strong lensing systems with multiple lens planes spread out across the distance between the lens and source, but these cases are relatively rare.}.



%The survey will produce the widest, deepest, and most uniform contiguous map in optical wavelengths of the southern sky, much of which has not been systematically surveyed---and not at such depth---until now. These features make DES suitable for finding many strong lensing systems that span large ranges in redshift and Einstein radii.  DES expects to uncover a large and diverse sample of strong gravitational lenses, which will provide for a rich science program. \end{rewrite}







%The DES data management (DESDM) team was responsible for the reduction of the Y1 images. The basic reductions and coadd source detection were performed by DESDM \citep{desai12, gruendl16} as described for the Y1A1  release\footnote{\url{http://data.darkenergysurvey.org/aux/releasenotes/DESDMrelease.html}}. 




%The characteristics will make it possible for DES to find a large number strong lenses --- not only of multiple scales (Einstein radii), but with sources of a variety of colors at high redshift. The ccds let us see redder adn higher redshift. The psf permits seeing radii down to a few arcseconds. 



%The only planned 1-hour integrations acquired with the R400 grating (Rank 1) were executed during the Priority Visiting Observer mode. The \nbpartial\ systems for which we did not obtain all planned exposures are missing the planned 3.7-hour R400 observations: in queue mode, these observations had lower Gemini observing priority. All planned 1-hour B600 observations were completed.



%\begin{itemize}
%\item General: lenses confirmed and not confirmed
%\item plot of images
%\item plot of spectra for confirmations
%\item table of lens information
%\item Compare mass modeling methods: einstein ring with better modeling
%\end{itemize}


This highlights the challenge of obtaining spectra for the very faint objects found in deep optical surveys: a great deal of integration time, in tandem with IR spectrographs, may be required to confirm the large lens samples predicted in current and future large surveys. The candidates that were ruled out as lensing systems indeed exhibit suggestive morphological features, but the candidate lensed sources were determined to be foreground galaxies through spectroscopic analysis.


 We estimate the Einstein radius (or radii if there is more than one source) by manually fitting a circle that passes through one or more spectroscopically confirmed features. The center is chosen to be the center of curvature of the candidate arc image(s). 
 
 This disparity sets the Einstein radius as the dominant contributor to the uncertainty. In the estimate, the uncertainty arises from statistical variation of the source images radial position, with the assumption that the correct center is chosen, as defined in \citet{diehl17}. These uncertainties are estimated to be up to an arcsecond. The distances between the source and lens cause some variation in the relative contributions to uncertainties: smaller distances provide for a greater contribution from the angular diameter distance $\DLS$. 
 
 and the Gemini Science Archive\footnote{\url{http://www.cadc-ccda.hia-iha.nrc-cnrc.gc.ca/en/gsa/index.html}}
